Asymptotic Degree of Random Monomial Ideals

One of the fundamental invariants connecting algebra and geometry is the degree of an ideal. In this paper we derive the probabilistic behavior of degree with respect to the versatile Erd\H{o}s-R\'enyi-type model for random monomial ideals defined in \cite{rmi}. We study the staircase structure associated to a monomial ideal, and show that in the random case the shape of the staircase diagram is approximately hyperbolic, and this behavior is robust across several random models. Since the discrete volume under this staircase is related to the summatory higher-order divisor function studied in number theory, we use this connection and our control over the shape of the staircase diagram to derive the asymptotic degree of a random monomial ideal. Another way to compute the degree of a monomial ideal is with a standard pair decomposition. This paper derives bounds on the number of standard pairs of a random monomial ideal indexed by any subset of the ring variables. The standard pairs indexed by maximal subsets give a count of degree, as well as being a more nuanced invariant of the random monomial ideal.

==> a-deg.tex <==
\begin{cor}
  There exists $C>0$ such that
  \[\expect{\adeg(\rmi)}=\Theta(Z_{1/p})\]
\end{cor}
\begin{proof}
  Since the arithmetic degree for a monomial ideal is given by the number of standard pairs, this is a clear corollary of Theorem~\ref{thm:sp-expected-value}
\end{proof}

==> conclusion.tex <==
\subsection{Arithmetic degree}

\subsection{Hilbert polynomial}


%In order to define what ``expected" means in this context, we must define a reasonable measure on the space of monomial ideals. There are several reasonable but distinct choices for such a measure (maybe describe these), and no reason to expect that these would lead to the same notion of ``expected Hilbert polynomial."




==> hilbert-poly.tex <==

Using the results about standard pairs, we can give the structure of the Hilbert Polynomial of a random monomial ideal.

\begin{thm}
  Hilbert polynomial
\end{thm}
\begin{proof}
  Notice that given the standard pairs of a monomial ideal, we can compute the hilbert polynomial as follows

  \[
  HP_{S/I}(t) = \sum_{(x^{\alpha},S)\text{ standard pairs of } I}\binom{t-\left|\alpha\right|+\left|S\right|-1}{\left|S\right|-1}
  \]

  Now for a random monomial ideal, notice that for $D\gg 0$, and a fixed support $S$, $\left|\alpha\right|>\left|S\right|$ for most standard pairs.


  Next notice that for fixed $b$ and $a<0$ , in $\binom{t+a}{b}$, the degree $k$ coefficient is $O(a^{b-k})$

  let $l(n)$, be the average value of $\left|\alpha\right|$ for standard pairs with $\left|S\right|=n$
  
  Thus
  \begin{align*}
    \left[HP_{S/I}\right]_k &= \sum_{(x^{\alpha},S)} O((-\left|\alpha\right|)^{\left|S\right|-1-k})\\
    &= \sum_{m=k+1}^{n} \left|sp(I,m)\right|O((-l(n))^{m-1-k})\\
    &= \sum_{m=k+1}^{n} \Theta(Z_{D^{-m}/p})O((-l(n))^{m-1-k})
  \end{align*}
  This should be dominated by m=k+1

  
  in particular, let $sp(\rmi,S)$ be the standard pairs of support $S$ for $\rmi$. Then ...
\end{proof}

